Automatic adaptation of object detectors to new domains using self-training

This work addresses the unsupervised adaptation of an existing object detector to a new target domain. We assume that a large number of unlabeled videos from this domain are readily available. We automatically obtain labels on the target data by using high-confidence detections from the existing detector, augmented with hard (misclassified) examples acquired by exploiting temporal cues using a tracker. These automatically-obtained labels are then used for re-training the original model. A modified knowledge distillation loss is proposed, and we investigate several ways of assigning soft-labels to the training examples from the target domain. Our approach is empirically evaluated on challenging face and pedestrian detection tasks: a face detector trained on WIDER-Face, which consists of high-quality images crawled from the web, is adapted to a large-scale surveillance data set; a pedestrian detector trained on clear, daytime images from the BDD-100K driving data set is adapted to all other scenarios such as rainy, foggy, night-time. Our results demonstrate the usefulness of incorporating hard examples obtained from tracking, the advantage of using soft-labels via distillation loss versus hard-labels, and show promising performance as a simple method for unsupervised domain adaptation of object detectors, with minimal dependence on hyper-parameters.

==> references <==
@article{schapire1998boosting,
  title={Boosting the margin: A new explanation for the effectiveness of voting methods},
  author={Schapire, Robert E and Freund, Yoav and Bartlett, Peter and Lee, Wee Sun and others},
  journal={The annals of statistics},
  volume={26},
  number={5},
  pages={1651--1686},
  year={1998},
  publisher={Institute of Mathematical Statistics}
}

@article{weinshall2018theory,
  title={Theory of Curriculum Learning, with Convex Loss Functions},
  author={Weinshall, Daphna and Amir, Dan},
  journal={arXiv preprint arXiv:1812.03472},
  year={2018}
}


@inproceedings{chen2018domain,
  title={Domain Adaptive Faster R-CNN for Object Detection in the Wild},
  author={Chen, Yuhua and Li, Wen and Sakaridis, Christos and Dai, Dengxin and Van Gool, Luc},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={3339--3348},
  year={2018}
}

@inproceedings{inoue2018cross,
  title={Cross-Domain Weakly-Supervised Object Detection Through Progressive Domain Adaptation},
  author={Inoue, Naoto and Furuta, Ryosuke and Yamasaki, Toshihiko and Aizawa, Kiyoharu},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={5001--5009},
  year={2018}
}

@inproceedings{xu2014incremental,
  title={Incremental Domain Adaptation of Deformable Part-based Models.},
  author={Xu, Jiaolong and Ramos, Sebastian and V{\'a}zquez, David and L{\'o}pez, Antonio M},
  booktitle = {Proceedings of the British Machine Vision Conference ({BMVC})},
  year = {2014}
}

@article{raj2015subspace,
  title={Subspace alignment based domain adaptation for rcnn detector},
  author={Raj, Anant and Namboodiri, Vinay P and Tuytelaars, Tinne},
  booktitle = {Proceedings of the British Machine Vision Conference ({BMVC})},
  year={2015}
}

@article{csurka2017domain,
  title={Domain adaptation for visual applications: A comprehensive survey},
  author={Csurka, Gabriela},
  journal={arXiv preprint arXiv:1702.05374},
  year={2017}
}

@inproceedings{ChenWW018,
  title     = {{LSTD:} {A} Low-Shot Transfer Detector for Object Detection},
  author    = {Hao Chen and
               Yali Wang and
               Guoyou Wang and
               Yu Qiao},
  booktitle = {{AAAI}},
  publisher = {{AAAI} Press},
  year      = {2018}
}

@inproceedings{chandaadapting,
  title={Adapting Object Detectors from Images to Weakly Labeled Videos},
  author={Chanda, Omit and Teh, Eu Wern and Rochan, Mrigank and Guo, Zhenyu and Wang, Yang},
  booktitle = {Proceedings of the British Machine Vision Conference ({BMVC})},
  year={2017}
}

@inproceedings{tang2012shifting,
  title={Shifting weights: Adapting object detectors from image to video},
  author={Tang, Kevin and Ramanathan, Vignesh and Fei-Fei, Li and Koller, Daphne},
  booktitle={Advances in Neural Information Processing Systems},
  pages={638--646},
  year={2012}
}

@inproceedings{mirrashed2013domain,
  title={Domain adaptive object detection},
  author={Mirrashed, Fatemeh and Morariu, Vlad I and Siddiquie, Behjat and Feris, Rogerio S and Davis, Larry S},
  booktitle={Applications of Computer Vision (WACV), 2013 IEEE Workshop on},
  pages={323--330},
  year={2013},
  organization={IEEE}
}

@inproceedings{htike2014unsupervised,
  title={Unsupervised detector adaptation by joint dataset feature learning},
  author={Htike, Kyaw Kyaw and Hogg, David},
  booktitle={International Conference on Computer Vision and Graphics},
  pages={270--277},
  year={2014},
  organization={Springer}
}

@article{shan2018pixel,
  title={Pixel and Feature Level Based Domain Adaption for Object Detection in Autonomous Driving},
  author={Shan, Yuhu and Lu, Wen Feng and Chew, Chee Meng},
  journal={arXiv preprint arXiv:1810.00345},
  year={2018}
}

@inproceedings{kuznetsova2015expanding,
  title={Expanding object detector's horizon: incremental learning framework for object detection in videos},
  author={Kuznetsova, Alina and Ju Hwang, Sung and Rosenhahn, Bodo and Sigal, Leonid},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={28--36},
  year={2015}
}

@inproceedings{jiang2016trajectory,
  title={A trajectory-based approach for object detection from video},
  author={Jiang, Chunhui and Li, Guiying and Liu, Junlong and Liu, Yunfeng and Tang, Ke},
  booktitle={Neural Networks (IJCNN), 2016 International Joint Conference on},
  pages={2887--2893},
  year={2016},
  organization={IEEE}
}

@article{kalogeiton2016analysing,
  title={Analysing domain shift factors between videos and images for object detection},
  author={Kalogeiton, Vicky and Ferrari, Vittorio and Schmid, Cordelia},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume={38},
  number={11},
  pages={2327--2334},
  year={2016}
}

@InProceedings{Jamal2018CVPR,
author = {Abdullah Jamal, Muhammad and Li, Haoxiang and Gong, Boqing},
title = {Deep Face Detector Adaptation Without Negative Transfer or Catastrophic Forgetting},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2018}
}

@inproceedings{hoffman2015detector,
  title={Detector discovery in the wild: Joint multiple instance and representation learning},
  author={Hoffman, Judy and Pathak, Deepak and Darrell, Trevor and Saenko, Kate},
  booktitle={Proceedings of the ieee conference on computer vision and pattern recognition},
  pages={2883--2891},
  year={2015}
}

@inproceedings{luo2017label,
  title={Label efficient learning of transferable representations acrosss domains and tasks},
  author={Luo, Zelun and Zou, Yuliang and Hoffman, Judy and Fei-Fei, Li F},
  booktitle={Advances in Neural Information Processing Systems},
  pages={165--177},
  year={2017}
}

@article{majumdarunsupervised,
  title={Unsupervised domain adaptation of deep object detectors},
  author={Majumdar, Debjeet and Namboodiri, Vinay P},
  booktitle={European Symposium on Artificial Neural Networks, Computational Intelligence and Machine Learning (ESANN)},
  year={2018}
}




@inproceedings{erdosrenyi,
  author    = {SouYoung Jin and 
  			   Hang Su and 
               Chris Stauffer and 
               Erik Learned-Miller},
  title		= {End-to-end face detection and cast grouping in movies using Erdos-Renyi clustering},
  booktitle = {ICCV}, 
  year 		= {2017}
}

@inproceedings{szegedy14adversarial,
  author    = {Christian Szegedy and
  			   Wojciech Zaremba and 
               Ilya Sutskever and
               Joan Bruna and
               Dumitru Erhan and
               Ian Goodfellow and
               Rob Fergus},
  title     = {Intriguing properties of neural networks},
  booktitle = {ICLR},
  pages     = {},
  year      = {2014},
  crossref  = {},
  url       = {},
  timestamp = {},
  biburl    = {},
  bibsource = {}
}

@inproceedings{ren15faster,
  author    = {Shaoqing Ren and
               Kaiming He and
               Ross B. Girshick and
               Jian Sun},
  title     = {Faster {R-CNN:} Towards Real-Time Object Detection with Region Proposal
               Networks},
  booktitle = {NIPS},
  pages     = {91--99},
  year      = {2015},
  crossref  = {DBLP:conf/nips/2015},
  url       = {http://papers.nips.cc/paper/5638-faster-r-cnn-towards-real-time-object-detection-with-region-proposal-networks},
  timestamp = {Fri, 08 Apr 2016 19:32:53 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/nips/RenHGS15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{ren16faster,
  author    = {Shaoqing Ren and
               Kaiming He and
               Ross Girshick and
               Jian Sun},
  title     = {Faster {R-CNN}: Towards Real-Time Object Detection with Region Proposal Networks},
  journal = {{IEEE} Trans. Pattern Anal. Mach. Intell.},
  year      = {2016}
}

@inproceedings{yang16wider,
  author    = {Shuo Yang and
               Ping Luo and
               Chen Change Loy and
               Xiaoou Tang},
  title     = {{WIDER FACE}: A Face Detection Benchmark},
  booktitle = {CVPR},
  year      = {2016}
}

@article{dollar15fast,
  author    = {Piotr Doll{\'{a}}r and
               C. Lawrence Zitnick},
  title     = {Fast Edge Detection Using Structured Forests},
  journal   = {{IEEE} Trans. Pattern Anal. Mach. Intell.},
  volume    = {37},
  number    = {8},
  pages     = {1558--1570},
  year      = {2015},
  url       = {http://dx.doi.org/10.1109/TPAMI.2014.2377715},
  doi       = {10.1109/TPAMI.2014.2377715},
  timestamp = {Sat, 12 Mar 2016 09:04:02 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/pami/DollarZ15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{zitnick2014edge,
  title={Edge boxes: Locating object proposals from edges},
  author={Zitnick, C Lawrence and Doll{\'a}r, Piotr},
  booktitle={European Conference on Computer Vision},
  pages={391--405},
  year={2014},
  organization={Springer}
}


@inproceedings{yang15from,
  author    = {Shuo Yang and
               Ping Luo and
               Chen Change Loy and
               Xiaoou Tang},
  title     = {From Facial Parts Responses to Face Detection: {A} Deep Learning Approach},
  booktitle = {ICCV},
  pages     = {3676--3684},
  year      = {2015},
  crossref  = {DBLP:conf/iccv/2015},
  url       = {http://dx.doi.org/10.1109/ICCV.2015.419},
  doi       = {10.1109/ICCV.2015.419},
  timestamp = {Thu, 12 May 2016 10:41:46 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/iccv/YangLLT15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{kuo15deepbox,
  author    = {Weicheng Kuo and
               Bharath Hariharan and
               Jitendra Malik},
  title     = {DeepBox: Learning Objectness with Convolutional Networks},
  booktitle = {ICCV},
  pages     = {2479--2487},
  year      = {2015},
  crossref  = {DBLP:conf/iccv/2015},
  url       = {http://dx.doi.org/10.1109/ICCV.2015.285},
  doi       = {10.1109/ICCV.2015.285},
  timestamp = {Thu, 12 May 2016 10:41:46 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/iccv/KuoHM15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{lin2014microsoft,
  title={Microsoft coco: Common objects in context},
  author={Lin, Tsung-Yi and Maire, Michael and Belongie, Serge and Hays, James and Perona, Pietro and Ramanan, Deva and Doll{\'a}r, Piotr and Zitnick, C Lawrence},
  booktitle={European conference on computer vision},
  pages={740--755},
  year={2014},
  organization={Springer}
}

@article{Dollar2012PAMI,
  author = {Piotr Doll\'ar and Christian Wojek and Bernt Schiele and Pietro Perona},
  title = {Pedestrian Detection: An Evaluation of the State of the Art},
  journal = {PAMI},
  volume = {34},
  year = {2012},
}


@Article{Everingham10,
   author = "Everingham, M. and Van~Gool, L. and Williams, C. K. I. and Winn, J. and Zisserman, A.",
   title = "The Pascal Visual Object Classes (VOC) Challenge",
   journal = "International Journal of Computer Vision",
   volume = "88",
   year = "2010",
   number = "2",
   month = jun,
   pages = "303--338",
} 


@inproceedings{Fouhey17b,
    title = {From Lifestyle VLOGs to Everyday Interactions},
    author = {David F. Fouhey and Weicheng Kuo and Alexei A. Efros and Jitendra Malik},
    booktitle = {Arxiv},
    year = {2017},
}	


@inproceedings{redmon2016you,
  title={You only look once: Unified, real-time object detection},
  author={Redmon, Joseph and Divvala, Santosh and Girshick, Ross and Farhadi, Ali},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={779--788},
  year={2016}
}

@inproceedings{liu2016ssd,
  title={Ssd: Single shot multibox detector},
  author={Liu, Wei and Anguelov, Dragomir and Erhan, Dumitru and Szegedy, Christian and Reed, Scott and Fu, Cheng-Yang and Berg, Alexander C},
  booktitle={European conference on computer vision},
  pages={21--37},
  year={2016},
  organization={Springer}
}


@inproceedings{cai2016unified,
  title={A unified multi-scale deep convolutional neural network for fast object detection},
  author={Cai, Zhaowei and Fan, Quanfu and Feris, Rogerio S and Vasconcelos, Nuno},
  booktitle={European Conference on Computer Vision},
  pages={354--370},
  year={2016},
  organization={Springer}
}


@article{lin2017focal,
  title={Focal loss for dense object detection},
  author={Lin, Tsung-Yi and Goyal, Priya and Girshick, Ross and He, Kaiming and Doll{\'a}r, Piotr},
  journal={arXiv preprint arXiv:1708.02002},
  year={2017}
}


@inproceedings{lin2017feature,
  title={Feature pyramid networks for object detection},
  author={Lin, Tsung-Yi and Doll{\'a}r, Piotr and Girshick, Ross and He, Kaiming and Hariharan, Bharath and Belongie, Serge},
  booktitle={CVPR},
  volume={1},
  number={2},
  pages={4},
  year={2017}
}



@article{sermanet2013overfeat,
  title={Overfeat: Integrated recognition, localization and detection using convolutional networks},
  author={Sermanet, Pierre and Eigen, David and Zhang, Xiang and Mathieu, Micha{\"e}l and Fergus, Rob and LeCun, Yann},
  journal={arXiv preprint arXiv:1312.6229},
  year={2013}
}

@inproceedings{girshick14rich,
  author    = {Ross B. Girshick and
               Jeff Donahue and
               Trevor Darrell and
               Jitendra Malik},
  title     = {Rich Feature Hierarchies for Accurate Object Detection and Semantic
               Segmentation},
  booktitle = {CVPR},
  pages     = {580--587},
  year      = {2014},
  crossref  = {DBLP:conf/cvpr/2014},
  url       = {http://dx.doi.org/10.1109/CVPR.2014.81},
  doi       = {10.1109/CVPR.2014.81},
  timestamp = {Thu, 28 Apr 2016 10:52:27 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/cvpr/GirshickDDM14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{krizhevsky12imagenet,
  author    = {Alex Krizhevsky and
               Ilya Sutskever and
               Geoffrey E. Hinton},
  title     = {ImageNet Classification with Deep Convolutional Neural Networks},
  booktitle = {NIPS},
  pages     = {1106--1114},
  year      = {2012},
  crossref  = {DBLP:conf/nips/2012},
  url       = {http://papers.nips.cc/paper/4824-imagenet-classification-with-deep-convolutional-neural-networks},
  timestamp = {Thu, 11 Dec 2014 17:34:07 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/nips/KrizhevskySH12},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{shrivastava2016training,
  title={Training region-based object detectors with online hard example mining},
  author={Shrivastava, Abhinav and Gupta, Abhinav and Girshick, Ross},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={761--769},
  year={2016}
}




@article{uijlings13selective,
  author    = {Jasper R. R. Uijlings and
               Koen E. A. van de Sande and
               Theo Gevers and
               Arnold W. M. Smeulders},
  title     = {Selective Search for Object Recognition},
  journal   = {International Journal of Computer Vision},
  volume    = {104},
  number    = {2},
  pages     = {154--171},
  year      = {2013},
  url       = {http://dx.doi.org/10.1007/s11263-013-0620-5},
  doi       = {10.1007/s11263-013-0620-5},
  timestamp = {Wed, 28 Aug 2013 13:53:08 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/ijcv/UijlingsSGS13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{he14spatial,
  author    = {Kaiming He and
               Xiangyu Zhang and
               Shaoqing Ren and
               Jian Sun},
  title     = {Spatial Pyramid Pooling in Deep Convolutional Networks for Visual
               Recognition},
  booktitle = {ECCV},
  pages     = {346--361},
  year      = {2014},
  crossref  = {DBLP:conf/eccv/2014-3},
  timestamp = {Tue, 09 Sep 2014 15:16:09 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/eccv/HeZR014},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{girshick15fast,
  author    = {Ross B. Girshick},
  title     = {Fast {R-CNN}},
  booktitle = {ICCV},
  pages     = {1440--1448},
  year      = {2015},
  crossref  = {DBLP:conf/iccv/2015},
  url       = {http://dx.doi.org/10.1109/ICCV.2015.169},
  doi       = {10.1109/ICCV.2015.169},
  timestamp = {Thu, 12 May 2016 10:41:46 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/iccv/Girshick15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{simonyan14very,
  author    = {Karen Simonyan and
               Andrew Zisserman},
  title     = {Very Deep Convolutional Networks for Large-Scale Image Recognition},
  journal   = {CoRR},
  volume    = {abs/1409.1556},
  year      = {2014},
  url       = {http://arxiv.org/abs/1409.1556},
  timestamp = {Wed, 01 Oct 2014 15:00:05 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/SimonyanZ14a},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@TechReport{fddbTech,
  author = {Vidit Jain and Erik Learned-Miller},
  title =  {{FDDB}: A Benchmark for Face Detection in Unconstrained Settings},
  institution =  {University of Massachusetts, Amherst},
  year = {2010},
  number = {UM-CS-2010-009}
  }

@inproceedings{klare15pushing,
  author    = {Brendan F. Klare and
               Ben Klein and
               Emma Taborsky and
               Austin Blanton and
               Jordan Cheney and
               Kristen Allen and
               Patrick Grother and
               Alan Mah and
               Mark Burge and
               Anil K. Jain},
  title     = {Pushing the frontiers of unconstrained face detection and recognition:
               {IARPA} {Janus} Benchmark {A}},
  booktitle = {CVPR},
  pages     = {1931--1939},
  year      = {2015},
  crossref  = {DBLP:conf/cvpr/2015},
  url       = {http://dx.doi.org/10.1109/CVPR.2015.7298803},
  doi       = {10.1109/CVPR.2015.7298803},
  timestamp = {Thu, 28 Apr 2016 16:31:13 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/cvpr/KlareKTBCAGMBJ15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{cheney15unconstrained,
  author    = {Jordan Cheney and
               Benjamin Klein and
               Anil K. Jain and
               Brendan F. Klare},
  title     = {Unconstrained face detection: State of the art baseline and challenges},
  booktitle = {ICB},
  pages     = {229--236},
  year      = {2015},
  crossref  = {DBLP:conf/icb/2015},
  url       = {http://dx.doi.org/10.1109/ICB.2015.7139089},
  doi       = {10.1109/ICB.2015.7139089},
  timestamp = {Mon, 13 Jul 2015 16:39:42 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/icb/CheneyKJK15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{ghiasi14occlusion,
  author    = {Golnaz Ghiasi and
               Charless C. Fowlkes},
  title     = {Occlusion Coherence: Localizing Occluded Faces with a Hierarchical
               Deformable Part Model},
  booktitle = {CVPR},
  pages     = {1899--1906},
  year      = {2014},
  crossref  = {DBLP:conf/cvpr/2014},
  url       = {http://dx.doi.org/10.1109/CVPR.2014.306},
  doi       = {10.1109/CVPR.2014.306},
  timestamp = {Thu, 28 Apr 2016 10:52:27 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/cvpr/GhiasiF14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{viola04robust,
  author    = {Paul A. Viola and
               Michael J. Jones},
  title     = {Robust Real-Time Face Detection},
  journal   = {International Journal of Computer Vision},
  volume    = {57},
  number    = {2},
  pages     = {137--154},
  year      = {2004},
  url       = {http://dx.doi.org/10.1023/B:VISI.0000013087.49260.fb},
  doi       = {10.1023/B:VISI.0000013087.49260.fb},
  timestamp = {Mon, 25 Apr 2005 11:01:56 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/ijcv/ViolaJ04},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{felzenszwalb10object,
  author    = {Pedro F. Felzenszwalb and
               Ross B. Girshick and
               David A. McAllester and
               Deva Ramanan},
  title     = {Object Detection with Discriminatively Trained Part-Based Models},
  journal   = {{IEEE} Trans. Pattern Anal. Mach. Intell.},
  volume    = {32},
  number    = {9},
  pages     = {1627--1645},
  year      = {2010},
  url       = {http://dx.doi.org/10.1109/TPAMI.2009.167},
  doi       = {10.1109/TPAMI.2009.167},
  timestamp = {Sat, 12 Mar 2016 09:04:02 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/pami/FelzenszwalbGMR10},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{ahonen06face,
  author    = {Timo Ahonen and
               Abdenour Hadid and
               Matti Pietik{\"{a}}inen},
  title     = {Face Description with Local Binary Patterns: Application to Face Recognition},
  journal   = {{IEEE} Trans. Pattern Anal. Mach. Intell.},
  volume    = {28},
  number    = {12},
  pages     = {2037--2041},
  year      = {2006},
  url       = {http://dx.doi.org/10.1109/TPAMI.2006.244},
  doi       = {10.1109/TPAMI.2006.244},
  timestamp = {Sat, 12 Mar 2016 09:03:59 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/pami/AhonenHP06},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{bay08speeded,
  author    = {Herbert Bay and
               Andreas Ess and
               Tinne Tuytelaars and
               Luc J. Van Gool},
  title     = {Speeded-Up Robust Features {(SURF)}},
  journal   = {Computer Vision and Image Understanding},
  volume    = {110},
  number    = {3},
  pages     = {346--359},
  year      = {2008},
  url       = {http://dx.doi.org/10.1016/j.cviu.2007.09.014},
  doi       = {10.1016/j.cviu.2007.09.014},
  timestamp = {Wed, 29 Oct 2008 20:58:33 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/cviu/BayETG08},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{dalal05histograms,
  author    = {Navneet Dalal and
               Bill Triggs},
  title     = {Histograms of Oriented Gradients for Human Detection},
  booktitle = {CVPR},
  pages     = {886--893},
  year      = {2005},
  crossref  = {DBLP:conf/cvpr/2005},
  url       = {http://dx.doi.org/10.1109/CVPR.2005.177},
  doi       = {10.1109/CVPR.2005.177},
  timestamp = {Thu, 23 Jun 2016 15:53:27 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/cvpr/DalalT05},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{dollar2009integral,
  title={Integral channel features},
  author={Doll{\'a}r, Piotr and Tu, Zhuowen and Perona, Pietro and Belongie, Serge},
  year={2009},
  publisher={BMVC Press}
}

@inproceedings{zitnick2014edge,
  title={Edge boxes: Locating object proposals from edges},
  author={Zitnick, C Lawrence and Doll{\'a}r, Piotr},
  booktitle={European Conference on Computer Vision},
  pages={391--405},
  year={2014},
  organization={Springer}
}

@article{mazeiarpa,
  title={IARPA Janus Benchmark--C: Face Dataset and Protocol},
  author={Maze, Brianna and Adams, Jocelyn and Duncan, James A and Kalka, Nathan and Miller, Tim and Otto, Charles and Jain, Anil K and Niggel, W Tyler and Anderson, Janet and Cheney, Jordan and others}
}

@inproceedings{ozerov2013evaluating,
  title={On evaluating face tracks in movies},
  author={Ozerov, Alexey and Vigouroux, Jean-Ronan and Chevallier, Louis and P{\'e}rez, Patrick},
  booktitle={Image Processing (ICIP), 2013 20th IEEE International Conference on},
  pages={3003--3007},
  year={2013},
  organization={IEEE}
}


@inproceedings{zhu12face,
  author    = {Xiangxin Zhu and
               Deva Ramanan},
  title     = {Face detection, pose estimation, and landmark localization in the
               wild},
  booktitle = {CVPR},
  pages     = {2879--2886},
  year      = {2012},
  crossref  = {DBLP:conf/cvpr/2012},
  url       = {http://dx.doi.org/10.1109/CVPR.2012.6248014},
  doi       = {10.1109/CVPR.2012.6248014},
  timestamp = {Tue, 25 Nov 2014 17:05:17 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/cvpr/ZhuR12},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{mathias14face,
  author    = {Markus Mathias and
               Rodrigo Benenson and
               Marco Pedersoli and
               Luc J. Van Gool},
  title     = {Face Detection without Bells and Whistles},
  booktitle = {ECCV},
  pages     = {720--735},
  year      = {2014},
  crossref  = {DBLP:conf/eccv/2014-4},
  url       = {http://dx.doi.org/10.1007/978-3-319-10593-2_47},
  doi       = {10.1007/978-3-319-10593-2_47},
  timestamp = {Tue, 26 Apr 2016 18:35:51 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/eccv/MathiasBPG14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{ghiasi14occlusion,
  author    = {Golnaz Ghiasi and
               Charless C. Fowlkes},
  title     = {Occlusion Coherence: Localizing Occluded Faces with a Hierarchical
               Deformable Part Model},
  booktitle = {CVPR},
  pages     = {1899--1906},
  year      = {2014},
  crossref  = {DBLP:conf/cvpr/2014},
  url       = {http://dx.doi.org/10.1109/CVPR.2014.306},
  doi       = {10.1109/CVPR.2014.306},
  timestamp = {Thu, 28 Apr 2016 10:52:27 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/cvpr/GhiasiF14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{chen14joint,
  author    = {Dong Chen and
               Shaoqing Ren and
               Yichen Wei and
               Xudong Cao and
               Jian Sun},
  title     = {Joint Cascade Face Detection and Alignment},
  booktitle = {ECCV},
  pages     = {109--122},
  year      = {2014},
  crossref  = {DBLP:conf/eccv/2014-6},
  url       = {http://dx.doi.org/10.1007/978-3-319-10599-4_8},
  doi       = {10.1007/978-3-319-10599-4_8},
  timestamp = {Mon, 06 Oct 2014 15:02:39 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/eccv/ChenRWCS14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{shen13detecting,
  author    = {Xiaohui Shen and
               Zhe Lin and
               Jonathan Brandt and
               Ying Wu},
  title     = {Detecting and Aligning Faces by Image Retrieval},
  booktitle = {CVPR},
  pages     = {3460--3467},
  year      = {2013},
  crossref  = {DBLP:conf/cvpr/2013},
  url       = {http://dx.doi.org/10.1109/CVPR.2013.444},
  doi       = {10.1109/CVPR.2013.444},
  timestamp = {Thu, 28 Apr 2016 10:52:27 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/cvpr/ShenLBW13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{li14efficient,
  author    = {Haoxiang Li and
               Zhe Lin and
               Jonathan Brandt and
               Xiaohui Shen and
               Gang Hua},
  title     = {Efficient Boosted Exemplar-Based Face Detection},
  booktitle = {CVPR},
  pages     = {1843--1850},
  year      = {2014},
  crossref  = {DBLP:conf/cvpr/2014},
  url       = {http://dx.doi.org/10.1109/CVPR.2014.238},
  doi       = {10.1109/CVPR.2014.238},
  timestamp = {Thu, 28 Apr 2016 10:52:27 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/cvpr/LiLBSH14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{vaillant-monrocq-lecun-94,
  author  =       "Vaillant, R. and Monrocq, C. and LeCun, Y.",
  title   =       "Original approach for the localisation of objects in images",
  journal =       "IEE Proc on Vision, Image, and Signal Processing",
  volume =        141,
  number =        4,
  pages =         "245-250",
  month =         "August",
  year =          1994,
}

@article{fowley98neural,
  author    = {Henry A. Rowley and
               Shumeet Baluja and
               Takeo Kanade},
  title     = {Neural Network-Based Face Detection},
  journal   = {{IEEE} Trans. Pattern Anal. Mach. Intell.},
  volume    = {20},
  number    = {1},
  pages     = {23--38},
  year      = {1998},
  url       = {http://dx.doi.org/10.1109/34.655647},
  doi       = {10.1109/34.655647},
  timestamp = {Sat, 12 Mar 2016 09:04:15 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/pami/RowleyBK98},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{osadchy07synergistic,
  author    = {Margarita Osadchy and
               Yann LeCun and
               Matthew L. Miller},
  title     = {Synergistic Face Detection and Pose Estimation with Energy-Based Models},
  journal   = {Journal of Machine Learning Research},
  volume    = {8},
  pages     = {1197--1215},
  year      = {2007},
  url       = {http://dl.acm.org/citation.cfm?id=1314539},
  timestamp = {Thu, 15 Dec 2011 15:52:06 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/jmlr/OsadchyLM07},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{ranjan15a,
  author = {Ranjan, Rajeev and Patel, Vishal M. and Chellappa, Rama},
  biburl = {http://www.bibsonomy.org/bibtex/257891faeda48e8517a900a420b710d8f/dblp},
  booktitle = {BTAS},
  crossref = {conf/btas/2015},
  ee = {http://dx.doi.org/10.1109/BTAS.2015.7358755},
  interhash = {cf94b7e2eb82101c276959211f8adda5},
  intrahash = {57891faeda48e8517a900a420b710d8f},
  isbn = {978-1-4799-8776-4},
  keywords = {dblp},
  pages = {1-8},
  publisher = {IEEE},
  timestamp = {2016-02-26T11:37:09.000+0100},
  title = {A deep pyramid Deformable Part Model for face detection.},
  url = {http://dblp.uni-trier.de/db/conf/btas/btas2015.html#RanjanPC15},
  year = 2015
}

@inproceedings{li15a,
  author    = {Haoxiang Li and
               Zhe Lin and
               Xiaohui Shen and
               Jonathan Brandt and
               Gang Hua},
  title     = {A convolutional neural network cascade for face detection},
  booktitle = {CVPR},
  pages     = {5325--5334},
  year      = {2015},
  crossref  = {DBLP:conf/cvpr/2015},
  url       = {http://dx.doi.org/10.1109/CVPR.2015.7299170},
  doi       = {10.1109/CVPR.2015.7299170},
  timestamp = {Thu, 28 Apr 2016 10:52:27 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/cvpr/LiLSBH15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{farfade15multi,
  author    = {Sachin Sudhakar Farfade and
               Mohammad J. Saberian and
               Li{-}Jia Li},
  title     = {Multi-view Face Detection Using Deep Convolutional Neural Networks},
  booktitle = {ICMR},
  pages     = {643--650},
  year      = {2015},
  crossref  = {DBLP:conf/mir/2015},
  url       = {http://doi.acm.org/10.1145/2671188.2749408},
  doi       = {10.1145/2671188.2749408},
  timestamp = {Wed, 29 Jul 2015 17:56:14 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/mir/FarfadeSL15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{li16face,
  author = {Li, Yunzhu and Sun, Benyuan and Wu, Tianfu and Wang, Yizhou and Gao, Wen},
  biburl = {http://www.bibsonomy.org/bibtex/22b5587016a9547fbf8353b7712aea367/dblp},
  ee = {http://arxiv.org/abs/1606.00850},
  interhash = {e1111841a4bd8869463894ba56487521},
  intrahash = {2b5587016a9547fbf8353b7712aea367},
  journal = {ECCV},
  keywords = {dblp},
  timestamp = {2016-07-02T11:37:10.000+0200},
  title = {Face Detection with End-to-End Integration of a ConvNet and a 3D Model.},
  url = {http://dblp.uni-trier.de/db/journals/corr/corr1606.html#LiSWW016},
  volume = {abs/1606.00850},
  year = 2016
}


@article{wang2017detecting,
  title={Detecting faces using region-based fully convolutional networks},
  author={Wang, Yitong and Ji, Xing and Zhou, Zheng and Wang, Hao and Li, Zhifeng},
  journal={arXiv preprint arXiv:1709.05256},
  year={2017}
}

@article{zhang2016joint,
  title={Joint face detection and alignment using multitask cascaded convolutional networks},
  author={Zhang, Kaipeng and Zhang, Zhanpeng and Li, Zhifeng and Qiao, Yu},
  journal={IEEE Signal Processing Letters},
  volume={23},
  number={10},
  pages={1499--1503},
  year={2016},
  publisher={IEEE}
}

@inproceedings{yu2016unitbox,
  title={Unitbox: An advanced object detection network},
  author={Yu, Jiahui and Jiang, Yuning and Wang, Zhangyang and Cao, Zhimin and Huang, Thomas},
  booktitle={Proceedings of the 2016 ACM on Multimedia Conference},
  pages={516--520},
  year={2016},
  organization={ACM}
}


@inproceedings{hu2017finding,
  title={Finding tiny faces},
  author={Hu, Peiyun and Ramanan, Deva},
  booktitle={2017 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={1522--1530},
  year={2017},
  organization={IEEE}
}


@article{wang2017detecting,
  title={Detecting faces using region-based fully convolutional networks},
  author={Wang, Yitong and Ji, Xing and Zhou, Zheng and Wang, Hao and Li, Zhifeng},
  journal={arXiv preprint arXiv:1709.05256},
  year={2017}
}

@inproceedings{dai2016r,
  title={R-fcn: Object detection via region-based fully convolutional networks},
  author={Dai, Jifeng and Li, Yi and He, Kaiming and Sun, Jian},
  booktitle={Advances in neural information processing systems},
  pages={379--387},
  year={2016}
}


@article{sun2017face,
  title={Face detection using deep learning: An improved faster rcnn approach},
  author={Sun, Xudong and Wu, Pengcheng and Hoi, Steven CH},
  journal={arXiv preprint arXiv:1701.08289},
  year={2017}
}


@article{wan2016bootstrapping,
  title={Bootstrapping face detection with hard negative examples},
  author={Wan, Shaohua and Chen, Zhijun and Zhang, Tao and Zhang, Bo and Wong, Kong-kat},
  journal={arXiv preprint arXiv:1608.02236},
  year={2016}
}


@inproceedings{dalal2005histograms,
  title={Histograms of oriented gradients for human detection},
  author={Dalal, Navneet and Triggs, Bill},
  booktitle={Computer Vision and Pattern Recognition, 2005. CVPR 2005. IEEE Computer Society Conference on},
  volume={1},
  pages={886--893},
  year={2005},
  organization={IEEE}
}

@article{sung1994learning,
  title={Learning and example selection for object and pattern detection},
  author={Sung, Kah-Kay and Poggio, Tomaso},
  booktitle={MIT A.I. Memp No. 1521},
  year={1994}
}

@article{felzenszwalb2010object,
  title={Object detection with discriminatively trained part-based models},
  author={Felzenszwalb, Pedro F and Girshick, Ross B and McAllester, David and Ramanan, Deva},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={32},
  number={9},
  pages={1627--1645},
  year={2010},
  publisher={IEEE}
}

@article{rowley1998neural,
  title={Neural network-based face detection},
  author={Rowley, Henry A and Baluja, Shumeet and Kanade, Takeo},
  journal={IEEE Transactions on pattern analysis and machine intelligence},
  volume={20},
  number={1},
  pages={23--38},
  year={1998},
  publisher={IEEE}
}


@article{friedman2000additive,
  title={Additive logistic regression: a statistical view of boosting (with discussion and a rejoinder by the authors)},
  author={Friedman, Jerome and Hastie, Trevor and Tibshirani, Robert and others},
  journal={The annals of statistics},
  volume={28},
  number={2},
  pages={337--407},
  year={2000},
  publisher={Institute of Mathematical Statistics}
}


@inproceedings{appel2013quickly,
  title={Quickly boosting decision trees--pruning underachieving features early},
  author={Appel, Ron and Fuchs, Thomas and Doll{\'a}r, Piotr and Perona, Pietro},
  booktitle={International Conference on Machine Learning},
  pages={594--602},
  year={2013}
}

@article{simo2014fracking,
  title={Fracking deep convolutional image descriptors},
  author={Simo-Serra, Edgar and Trulls, Eduard and Ferraz, Luis and Kokkinos, Iasonas and Moreno-Noguer, Francesc},
  journal={CoRR, abs/1412.6537},
  volume={2},
  year={2014}
}

@inproceedings{bromley1994signature,
  title={Signature verification using a" siamese" time delay neural network},
  author={Bromley, Jane and Guyon, Isabelle and LeCun, Yann and S{\"a}ckinger, Eduard and Shah, Roopak},
  booktitle={Advances in Neural Information Processing Systems},
  pages={737--744},
  year={1994}
}

@inproceedings{jiang2017face,
  title={Face detection with the faster R-CNN},
  author={Jiang, Huaizu and Learned-Miller, Erik},
  booktitle={Automatic Face \& Gesture Recognition (FG 2017), 2017 12th IEEE International Conference on},
  pages={650--657},
  year={2017},
  organization={IEEE}
}


@inproceedings{real2017youtube,
  title={Youtube-boundingboxes: A large high-precision human-annotated data set for object detection in video},
  author={Real, Esteban and Shlens, Jonathon and Mazzocchi, Stefano and Pan, Xin and Vanhoucke, Vincent},
  booktitle={2017 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={7464--7473},
  year={2017},
  organization={IEEE}
}

@book{scholkopf2001learning,
  title={Learning with kernels: support vector machines, regularization, optimization, and beyond},
  author={Scholkopf, Bernhard and Smola, Alexander J},
  year={2001},
  publisher={MIT press}
}


@article{westonlarge,
  title={Large-Scale Semi-Supervised Learning},
  author={WESTON, Jason}
}

@article{chapelle2009semi,
  title={Semi-supervised learning (chapelle, o. et al., eds.; 2006)[book reviews]},
  author={Chapelle, Olivier and Scholkopf, Bernhard and Zien, Alexander},
  journal={IEEE Transactions on Neural Networks},
  volume={20},
  number={3},
  pages={542--542},
  year={2009},
  publisher={IEEE}
}


@inproceedings{blum1998combining,
  title={Combining labeled and unlabeled data with co-training},
  author={Blum, Avrim and Mitchell, Tom},
  booktitle={Proceedings of the eleventh annual conference on Computational learning theory},
  pages={92--100},
  year={1998},
  organization={ACM}
}


@article{rosenberg2005semi,
  title={Semi-supervised self-training of object detection models},
  author={Rosenberg, Chuck and Hebert, Martial and Schneiderman, Henry},
  year={2005},
  publisher={IEEE Press}
}

@article{loshchilov2015online,
  title={Online batch selection for faster training of neural networks},
  author={Loshchilov, Ilya and Hutter, Frank},
  journal={arXiv preprint arXiv:1511.06343},
  year={2015}
}


@inproceedings{Laine2017, 
  author =    {Samuli Laine and Timo Aila},
  title =     {Temporal Ensembling for Semi-Supervised Learning},
  journal =   {Proc. International Conference on Learning Representations (ICLR)},
  year =      {2017},
}


@inproceedings{kalal2010pn,
  title={Pn learning: Bootstrapping binary classifiers by structural constraints},
  author={Kalal, Zdenek and Matas, Jiri and Mikolajczyk, Krystian},
  booktitle={Computer Vision and Pattern Recognition (CVPR), 2010 IEEE Conference on},
  pages={49--56},
  year={2010},
  organization={IEEE}
}


@article{abu2016youtube,
  title={Youtube-8m: A large-scale video classification benchmark},
  author={Abu-El-Haija, Sami and Kothari, Nisarg and Lee, Joonseok and Natsev, Paul and Toderici, George and Varadarajan, Balakrishnan and Vijayanarasimhan, Sudheendra},
  journal={arXiv preprint arXiv:1609.08675},
  year={2016}
}


@article{wang2017fast,
  title={A-fast-rcnn: Hard positive generation via adversary for object detection},
  author={Wang, Xiaolong and Shrivastava, Abhinav and Gupta, Abhinav},
  booktitle={2017 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2017},
  organization={IEEE}
}

@inproceedings{singh2016track,
  title={Track and Transfer: Watching Videos to Simulate Strong Human Supervision for Weakly-Supervised Object Detection.},
  author={Singh, Krishna Kumar and Xiao, Fanyi and Lee, Yong Jae},
  booktitle={CVPR},
  volume={1},
  pages={2},
  year={2016}
}

@article{zhang2017s,
  title={S3FD: Single Shot Scale-invariant Face Detector},
  author={Zhang, Shifeng and Zhu, Xiangyu and Lei, Zhen and Shi, Hailin and Wang, Xiaobo and Li, Stan Z},
  journal={arXiv preprint arXiv:1708.05237},
  year={2017}
}


% ---------------------------------------------------------------------------
% Active learning, SVMs
% ---------------------------------------------------------------------------
@book{scholkopf2002learning,
  title={Learning with kernels: support vector machines, regularization, optimization, and beyond},
  author={Sch{\"o}lkopf, Bernhard and Smola, Alexander J},
  year={2002},
  publisher={MIT press}
}

@inproceedings{chang2017active,
  title={Active Bias: Training More Accurate Neural Networks by Emphasizing High Variance Samples},
  author={Chang, Haw-Shiuan and Learned-Miller, Erik and McCallum, Andrew},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1003--1013},
  year={2017}
}

@article{settles1648active,
  title={Active Learning Literature Survey. 2010},
  author={Settles, Burr},
  journal={Computer Sciences Technical Report},
  volume={1648}
}

@inproceedings{schohn2000less,
  title={Less is more: Active learning with support vector machines},
  author={Schohn, Greg and Cohn, David},
  booktitle={ICML},
  pages={839--846},
  year={2000},
  organization={Citeseer}
}

@article{gao2015active,
  title={Active Sampler: Light-weight Accelerator for Complex Data Analytics at Scale},
  author={Gao, Jinyang and Jagadish, HV and Ooi, Beng Chin},
  journal={arXiv preprint arXiv:1512.03880},
  year={2015}
}

@inproceedings{geman1986markov,
  title={Markov random field image models and their applications to computer vision},
  author={Geman, Stuart and Graffigne, Christine},
  booktitle={Proceedings of the international congress of mathematicians},
  volume={1},
  pages={2},
  year={1986}
}

@book{sutton2006introduction,
  title={An introduction to conditional random fields for relational learning},
  author={Sutton, Charles and McCallum, Andrew},
  volume={2},
  year={2006},
  publisher={Introduction to statistical relational learning. MIT Press}
}

@inproceedings{stalder2010cascaded,
  title={Cascaded confidence filtering for improved tracking-by-detection},
  author={Stalder, Severin and Grabner, Helmut and Van Gool, Luc},
  booktitle={European Conference on Computer Vision},
  pages={369--382},
  year={2010},
  organization={Springer}
}

@inproceedings{klaser2010human,
  title={Human focused action localization in video},
  author={Kl{\"a}ser, Alexander and Marsza{\l}ek, Marcin and Schmid, Cordelia and Zisserman, Andrew},
  booktitle={European Conference on Computer Vision},
  pages={219--233},
  year={2010},
  organization={Springer}
}

@inproceedings{yang2012online,
  title={An online learned CRF model for multi-target tracking},
  author={Yang, Bo and Nevatia, Ram},
  booktitle={Computer Vision and Pattern Recognition (CVPR), 2012 IEEE Conference on},
  pages={2034--2041},
  year={2012},
  organization={IEEE}
}


% ---------------------------------------------------------------------------

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@inproceedings{szegedy2015going,
  title={Going deeper with convolutions},
  author={Szegedy, Christian and Liu, Wei and Jia, Yangqing and Sermanet, Pierre and Reed, Scott and Anguelov, Dragomir and Erhan, Dumitru and Vanhoucke, Vincent and Rabinovich, Andrew and others},
  year={2015},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
}

@Article{Simonyan14c,
    author       = "Simonyan, K. and Zisserman, A.",
    title        = "Very Deep Convolutional Networks for Large-Scale Image Recognition",
    journal      = "CoRR",
    volume       = "abs/1409.1556",
    year         = "2014"
}


% Adversarial examples

@article{szegedy2013intriguing,
  title={Intriguing properties of neural networks},
  author={Szegedy, Christian and Zaremba, Wojciech and Sutskever, Ilya and Bruna, Joan and Erhan, Dumitru and Goodfellow, Ian and Fergus, Rob},
  journal={arXiv preprint arXiv:1312.6199},
  year={2013}
}

@article{lu2017no,
  title={No need to worry about adversarial examples in object detection in autonomous vehicles},
  author={Lu, Jiajun and Sibai, Hussein and Fabry, Evan and Forsyth, David},
  journal={arXiv preprint arXiv:1707.03501},
  year={2017}
}

@article{luo2015foveation,
  title={Foveation-based mechanisms alleviate adversarial examples},
  author={Luo, Yan and Boix, Xavier and Roig, Gemma and Poggio, Tomaso and Zhao, Qi},
  journal={arXiv preprint arXiv:1511.06292},
  year={2015}
}

@article{athalye2017synthesizing,
  title={Synthesizing robust adversarial examples},
  author={Athalye, Anish and Sutskever, Ilya},
  journal={arXiv preprint arXiv:1707.07397},
  year={2017}
}






% ---------------------------------------------------------------------------
% Pedestrian detections
% ---------------------------------------------------------------------------

@inproceedings{dollar2009pedestrian,
  title={Pedestrian detection: A benchmark},
  author={Doll{\'a}r, Piotr and Wojek, Christian and Schiele, Bernt and Perona, Pietro},
  booktitle={Computer Vision and Pattern Recognition, 2009. CVPR 2009. IEEE Conference on},
  pages={304--311},
  year={2009},
  organization={IEEE}
}

@inproceedings{du2017fused,
  title={Fused DNN: A deep neural network fusion approach to fast and robust pedestrian detection},
  author={Du, Xianzhi and El-Khamy, Mostafa and Lee, Jungwon and Davis, Larry},
  booktitle={Applications of Computer Vision (WACV), 2017 IEEE Winter Conference on},
  pages={953--961},
  year={2017},
  organization={IEEE}
}

@inproceedings{cai2015learning,
  title={Learning complexity-aware cascades for deep pedestrian detection},
  author={Cai, Zhaowei and Saberian, Mohammad and Vasconcelos, Nuno},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={3361--3369},
  year={2015}
}

@inproceedings{hosang2015taking,
  title={Taking a deeper look at pedestrians},
  author={Hosang, Jan and Omran, Mohamed and Benenson, Rodrigo and Schiele, Bernt},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={4073--4082},
  year={2015}
}

@article{li2017scale,
  title={Scale-aware fast R-CNN for pedestrian detection},
  author={Li, Jianan and Liang, Xiaodan and Shen, ShengMei and Xu, Tingfa and Feng, Jiashi and Yan, Shuicheng},
  journal={IEEE Transactions on Multimedia},
  year={2017},
  publisher={IEEE}
}
 
@inproceedings{tian2015deep,
  title={Deep learning strong parts for pedestrian detection},
  author={Tian, Yonglong and Luo, Ping and Wang, Xiaogang and Tang, Xiaoou},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={1904--1912},
  year={2015}
}

@inproceedings{zhang2016faster,
  title={Is faster r-cnn doing well for pedestrian detection?},
  author={Zhang, Liliang and Lin, Liang and Liang, Xiaodan and He, Kaiming},
  booktitle={European Conference on Computer Vision},
  pages={443--457},
  year={2016},
  organization={Springer}
}

@inproceedings{zhang2016far,
  title={How far are we from solving pedestrian detection?},
  author={Zhang, Shanshan and Benenson, Rodrigo and Omran, Mohamed and Hosang, Jan and Schiele, Bernt},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={1259--1267},
  year={2016}
}


@article{odena2018realistic,
  title={Realistic Evaluation of Semi-Supervised Learning Algorithms},
  author={Odena, Augustus and Oliver, Avital and Raffel, Colin and Cubuk, Ekin Dogus and Goodfellow, Ian},
  year={2018}
}

@inproceedings{lee2013pseudo,
  title={Pseudo-label: The simple and efficient semi-supervised learning method for deep neural networks},
  author={Lee, Dong-Hyun},
  booktitle={ICML Workshop},
  volume={3},
  pages={2},
  year={2013}
}

@article{papadopoulos2017training,
  title={Training object class detectors with click supervision},
  author={Papadopoulos, Dim P and Uijlings, Jasper RR and Keller, Frank and Ferrari, Vittorio},
  journal={arXiv preprint arXiv:1704.06189},
  year={2017}
}

@article{brazil2017illuminating,
  title={Illuminating Pedestrians via Simultaneous Detection \& Segmentation},
  author={Brazil, Garrick and Yin, Xi and Liu, Xiaoming},
  journal={arXiv preprint arXiv:1706.08564},
  year={2017}
}

@inproceedings{najibi2017ssh,
title={{SSH}: Single Stage Headless Face Detector},
author={Najibi, Mahyar and Samangouei, Pouya and Chellappa, Rama and Davis, Larry},
booktitle={The IEEE International Conference on Computer Vision (ICCV)},
year={2017}
}

@InProceedings{Jamal_2018_CVPR,
author = {Abdullah Jamal, Muhammad and Li, Haoxiang and Gong, Boqing},
title = {Deep Face Detector Adaptation Without Negative Transfer or Catastrophic Forgetting},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2018}
}

@article{sonntag2017fine,
  title={Fine-tuning deep CNN models on specific MS COCO categories},
  author={Sonntag, Daniel and Barz, Michael and Zacharias, Jan and Stauden, Sven and Rahmani, Vahid and F{\'o}thi, {\'A}ron and L{\H{o}}rincz, Andr{\'a}s},
  journal={arXiv preprint arXiv:1709.01476},
  year={2017}
}

@inproceedings{tang2012shifting,
  title={Shifting weights: Adapting object detectors from image to video},
  author={Tang, Kevin and Ramanathan, Vignesh and Fei-Fei, Li and Koller, Daphne},
  booktitle={Advances in Neural Information Processing Systems},
  pages={638--646},
  year={2012}
}

@inproceedings{kendall2017uncertainties,
  title={What uncertainties do we need in bayesian deep learning for computer vision?},
  author={Kendall, Alex and Gal, Yarin},
  booktitle={Advances in neural information processing systems},
  pages={5574--5584},
  year={2017}
}

@inproceedings{novotny2018self,
  title={Self-supervised Learning of Geometrically Stable Features Through Probabilistic Introspection},
  author={Novotny, David and Albanie, Samuel and Larlus, Diane and Vedaldi, Andrea},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={3637--3645},
  year={2018}
}

@inproceedings{chen2017learning,
  title={Learning efficient object detection models with knowledge distillation},
  author={Chen, Guobin and Choi, Wongun and Yu, Xiang and Han, Tony and Chandraker, Manmohan},
  booktitle={Advances in Neural Information Processing Systems},
  pages={742--751},
  year={2017}
}

@article{triguero2015self,
  title={Self-labeled techniques for semi-supervised learning: taxonomy, software and empirical study},
  author={Triguero, Isaac and Garc{\'\i}a, Salvador and Herrera, Francisco},
  journal={Knowledge and Information Systems},
  volume={42},
  number={2},
  pages={245--284},
  year={2015},
  publisher={Springer}
}

@inproceedings{li2005setred,
  title={SETRED: self-training with editing},
  author={Li, Ming and Zhou, Zhi-Hua},
  booktitle={Pacific-Asia Conference on Knowledge Discovery and Data Mining},
  pages={611--621},
  year={2005},
  organization={Springer}
}

@article{muhlenbach2004identifying,
  title={Identifying and handling mislabelled instances},
  author={Muhlenbach, Fabrice and Lallich, St{\'e}phane and Zighed, Djamel A},
  journal={Journal of Intelligent Information Systems},
  volume={22},
  number={1},
  pages={89--109},
  year={2004},
  publisher={Springer}
}

@inproceedings{jiang2004editing,
  title={Editing training data for kNN classifiers with neural network ensemble},
  author={Jiang, Yuan and Zhou, Zhi-Hua},
  booktitle={International symposium on neural networks},
  pages={356--361},
  year={2004},
  organization={Springer}
}

@article{wilson1972asymptotic,
  title={Asymptotic properties of nearest neighbor rules using edited data},
  author={Wilson, Dennis L},
  journal={IEEE Transactions on Systems, Man, and Cybernetics},
  number={3},
  pages={408--421},
  year={1972},
  publisher={Citeseer}
}

@inproceedings{nam2016learning,
  title={Learning multi-domain convolutional neural networks for visual tracking},
  author={Nam, Hyeonseob and Han, Bohyung},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={4293--4302},
  year={2016}
}

@inproceedings{jin2018unsup,
    Author = {SouYoung Jin and Aruni RoyChowdhury and Huaizu Jiang and Ashish Singh and Aditya Prasad and Deep Chakraborty and Erik Learned-Miller},
    Title = {Unsupervised Hard Example Mining from Videos for Improved Object Detection},
    Booktitle = {European Conference on Computer Vision (ECCV)},
    Year = {2018}
}

@article{kalkaijb,
  title={IJB--S: IARPA Janus Surveillance Video Benchmark},
  author={Kalka, Nathan D and Maze, Brianna and Duncan, James A and O’Connor, Kevin and Elliott, Stephen and Hebert, Kaleb and Bryan, Julia and Jain, Anil K}
}

@article{yu2018bdd100k,
  title={BDD100K: A Diverse Driving Video Database with Scalable Annotation Tooling},
  author={Yu, Fisher and Xian, Wenqi and Chen, Yingying and Liu, Fangchen and Liao, Mike and Madhavan, Vashisht and Darrell, Trevor},
  journal={arXiv preprint arXiv:1805.04687},
  year={2018}
}

@InProceedings{inoue2018cross,
author = {Inoue, Naoto and Furuta, Ryosuke and Yamasaki, Toshihiko and Aizawa, Kiyoharu},
title = {Cross-Domain Weakly-Supervised Object Detection through Progressive Domain Adaptation},
booktitle = {CVPR},
year = {2018}
}

@InProceedings{zhu2017unpaired,
  title={Unpaired image-to-image translation using cycle-consistent adversarial networks},
  author={Zhu, Jun-Yan and Park, Taesung and Isola, Phillip and Efros, Alexei A},
  booktitle = {ICCV)},
  year={2017}
}

@inproceedings{chen2018domain,
  title={Domain adaptive faster r-cnn for object detection in the wild},
  author={Chen, Yuhua and Li, Wen and Sakaridis, Christos and Dai, Dengxin and Van Gool, Luc},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={3339--3348},
  year={2018}
}

@article{ganin2016domain,
  title={Domain-adversarial training of neural networks},
  author={Ganin, Yaroslav and Ustinova, Evgeniya and Ajakan, Hana and Germain, Pascal and Larochelle, Hugo and Laviolette, Fran{\c{c}}ois and Marchand, Mario and Lempitsky, Victor},
  journal={The Journal of Machine Learning Research},
  volume={17},
  number={1},
  pages={2096--2030},
  year={2016},
  publisher={JMLR. org}
}

@article{ganin2014unsupervised,
  title={Unsupervised domain adaptation by backpropagation},
  author={Ganin, Yaroslav and Lempitsky, Victor},
  journal={arXiv preprint arXiv:1409.7495},
  year={2014}
}

@inproceedings{rosenberg2005semi,
  title={Semi-Supervised Self-Training of Object Detection Models.},
  author={Rosenberg, Chuck and Hebert, Martial and Schneiderman, Henry},
  booktitle={WACV/MOTION},
  pages={29--36},
  year={2005}
}

@inproceedings{weber2000unsupervised,
  title={Unsupervised learning of models for recognition},
  author={Weber, Markus and Welling, Max and Perona, Pietro},
  booktitle={European conference on computer vision},
  pages={18--32},
  year={2000},
  organization={Springer}
}

@inproceedings{sharma2013efficient,
  title={Efficient detector adaptation for object detection in a video},
  author={Sharma, Pramod and Nevatia, Ram},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={3254--3261},
  year={2013}
}

@inproceedings{donahue2013semi,
  title={Semi-supervised domain adaptation with instance constraints},
  author={Donahue, Jeff and Hoffman, Judy and Rodner, Erik and Saenko, Kate and Darrell, Trevor},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={668--675},
  year={2013}
}

@inproceedings{han2012detection,
  title={Detection by detections: Non-parametric detector adaptation for a video},
  author={Han, TX and Hua, Gang and Wang, Xiaoyu},
  booktitle={2012 IEEE Conference on Computer Vision and Pattern Recognition},
  pages={350--357},
  year={2012},
  organization={IEEE}
}

@inproceedings{chandaadapting,
  title={Adapting Object Detectors from Images to Weakly Labeled Videos},
  author={Chanda, Omit and Teh, Eu Wern and Rochan, Mrigank and Guo, Zhenyu and Wang, Yang},
  booktitle={The 28th British Machine Vision Conference (BMVC)}
}

@inproceedings{baluja1999probabilistic,
  title={Probabilistic modeling for face orientation discrimination: Learning from labeled and unlabeled data},
  author={Baluja, Shumeet},
  booktitle={Advances in Neural Information Processing Systems},
  pages={854--860},
  year={1999}
}

@inproceedings{selinger2001minimally,
  title={Minimally supervised acquisition of 3D recognition models from cluttered images},
  author={Selinger, Andrea and Nelson, Randal C},
  booktitle={Computer Vision and Pattern Recognition, 2001. CVPR 2001. Proceedings of the 2001 IEEE Computer Society Conference on},
  volume={1},
  pages={I--I},
  year={2001},
  organization={IEEE}
}

@inproceedings{levin2003unsupervised,
  title={Unsupervised Improvement of Visual Detectors using Co-Training.},
  author={Levin, Anat and Viola, Paul A and Freund, Yoav},
  booktitle={ICCV},
  volume={1},
  pages={626--633},
  year={2003}
}

@inproceedings{fergus2003object,
  title={Object class recognition by unsupervised scale-invariant learning},
  author={Fergus, Robert and Perona, Pietro and Zisserman, Andrew},
  booktitle={Computer Vision and Pattern Recognition, 2003. Proceedings. 2003 IEEE Computer Society Conference on},
  volume={2},
  pages={II--II},
  year={2003},
  organization={IEEE}
}

@article{mahalanobis1930test,
  title={On test and measures of group divergence, Part I: Theoretical formulae},
  author={Mahalanobis, Prasanta Chandra},
  year={1930},
  publisher={Journal and Proceedings of Asiatic Society of Bengal New series26, 541-588}
}

@inproceedings{nigam2000analyzing,
  title={Analyzing the effectiveness and applicability of co-training},
  author={Nigam, Kamal and Ghani, Rayid},
  booktitle={Proceedings of the ninth international conference on Information and knowledge management},
  pages={86--93},
  year={2000},
  organization={ACM}
}

@article{reed2014training,
  title={Training deep neural networks on noisy labels with bootstrapping},
  author={Reed, Scott and Lee, Honglak and Anguelov, Dragomir and Szegedy, Christian and Erhan, Dumitru and Rabinovich, Andrew},
  journal={arXiv preprint arXiv:1412.6596},
  year={2014}
}

@article{sukhbaatar2014training,
  title={Training convolutional networks with noisy labels},
  author={Sukhbaatar, Sainbayar and Bruna, Joan and Paluri, Manohar and Bourdev, Lubomir and Fergus, Rob},
  journal={arXiv preprint arXiv:1406.2080},
  year={2014}
}

@inproceedings{natarajan2013learning,
  title={Learning with noisy labels},
  author={Natarajan, Nagarajan and Dhillon, Inderjit S and Ravikumar, Pradeep K and Tewari, Ambuj},
  booktitle={Advances in neural information processing systems},
  pages={1196--1204},
  year={2013}
}

@inproceedings{biggio2011support,
  title={Support vector machines under adversarial label noise},
  author={Biggio, Battista and Nelson, Blaine and Laskov, Pavel},
  booktitle={Asian Conference on Machine Learning},
  pages={97--112},
  year={2011}
}

@inproceedings{elkan2008learning,
  title={Learning classifiers from only positive and unlabeled data},
  author={Elkan, Charles and Noto, Keith},
  booktitle={Proceedings of the 14th ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={213--220},
  year={2008},
  organization={ACM}
}

@inproceedings{chen2015webly,
  title={Webly supervised learning of convolutional networks},
  author={Chen, Xinlei and Gupta, Abhinav},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={1431--1439},
  year={2015}
}


@inproceedings{patrini2017making,
  title={Making deep neural networks robust to label noise: A loss correction approach},
  author={Patrini, Giorgio and Rozza, Alessandro and Menon, Aditya Krishna and Nock, Richard and Qu, Lizhen},
  booktitle={Proc. IEEE Conf. Comput. Vis. Pattern Recognit.(CVPR)},
  pages={2233--2241},
  year={2017}
}

@inproceedings{li2017learning,
  title={Learning from Noisy Labels with Distillation.},
  author={Li, Yuncheng and Yang, Jianchao and Song, Yale and Cao, Liangliang and Luo, Jiebo and Li, Li-Jia},
  booktitle={ICCV},
  pages={1928--1936},
  year={2017}
}

@article{rolnick2017deep,
  title={Deep learning is robust to massive label noise},
  author={Rolnick, David and Veit, Andreas and Belongie, Serge and Shavit, Nir},
  journal={arXiv preprint arXiv:1705.10694},
  year={2017}
}

@book{sugiyama2017dataset,
  title={Dataset shift in machine learning},
  author={Sugiyama, Masashi and Lawrence, Neil D and Schwaighofer, Anton and others},
  year={2017},
  publisher={The MIT Press}
}

@inproceedings{gretton2008dataset,
  title={Dataset shift in machine learning},
  author={Gretton, A and Smola, A and Huang, J and Schmittfull, M and Borgwardt, K and Sch{\"o}lkopf, B},
  booktitle={Covariate Shift and Local Learning by Distribution Matching},
  pages={131--160},
  year={2008},
  organization={MIT Press}
}

@article{ben2010theory,
  title={A theory of learning from different domains},
  author={Ben-David, Shai and Blitzer, John and Crammer, Koby and Kulesza, Alex and Pereira, Fernando and Vaughan, Jennifer Wortman},
  journal={Machine learning},
  volume={79},
  number={1-2},
  pages={151--175},
  year={2010},
  publisher={Springer}
}

@article{radosavovic2017data,
  title={Data distillation: Towards omni-supervised learning},
  author={Radosavovic, Ilija and Doll{\'a}r, Piotr and Girshick, Ross and Gkioxari, Georgia and He, Kaiming},
  journal={arXiv preprint arXiv:1712.04440},
  year={2017}
}

@inproceedings{sun2016deep,
  title={Deep coral: Correlation alignment for deep domain adaptation},
  author={Sun, Baochen and Saenko, Kate},
  booktitle={European Conference on Computer Vision},
  pages={443--450},
  year={2016},
  organization={Springer}
}

@article{tzeng2014deep,
  title={Deep domain confusion: Maximizing for domain invariance},
  author={Tzeng, Eric and Hoffman, Judy and Zhang, Ning and Saenko, Kate and Darrell, Trevor},
  journal={arXiv preprint arXiv:1412.3474},
  year={2014}
}

@article{long2015learning,
  title={Learning transferable features with deep adaptation networks},
  author={Long, Mingsheng and Cao, Yue and Wang, Jianmin and Jordan, Michael I},
  journal={arXiv preprint arXiv:1502.02791},
  year={2015}
}

@inproceedings{tzeng2017adversarial,
  title={Adversarial discriminative domain adaptation},
  author={Tzeng, Eric and Hoffman, Judy and Saenko, Kate and Darrell, Trevor},
  booktitle={Computer Vision and Pattern Recognition (CVPR)},
  volume={1},
  number={2},
  pages={4},
  year={2017}
}

@inproceedings{tzeng2015simultaneous,
  title={Simultaneous deep transfer across domains and tasks},
  author={Tzeng, Eric and Hoffman, Judy and Darrell, Trevor and Saenko, Kate},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={4068--4076},
  year={2015}
}

@article{hoffman2017cycada,
  title={Cycada: Cycle-consistent adversarial domain adaptation},
  author={Hoffman, Judy and Tzeng, Eric and Park, Taesung and Zhu, Jun-Yan and Isola, Phillip and Saenko, Kate and Efros, Alexei A and Darrell, Trevor},
  journal={arXiv preprint arXiv:1711.03213},
  year={2017}
}

@inproceedings{bousmalis2017unsupervised,
  title={Unsupervised pixel-level domain adaptation with generative adversarial networks},
  author={Bousmalis, Konstantinos and Silberman, Nathan and Dohan, David and Erhan, Dumitru and Krishnan, Dilip},
  booktitle={The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  volume={1},
  number={2},
  pages={7},
  year={2017}
}

@inproceedings{hong2018conditional,
  title={Conditional Generative Adversarial Network for Structured Domain Adaptation},
  author={Hong, Weixiang and Wang, Zhenzhen and Yang, Ming and Yuan, Junsong},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={1335--1344},
  year={2018}
}

@inproceedings{hu2018duplex,
  title={Duplex Generative Adversarial Network for Unsupervised Domain Adaptation},
  author={Hu, Lanqing and Kan, Meina and Shan, Shiguang and Chen, Xilin},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={1498--1507},
  year={2018}
}

@misc{Detectron2018,
  author =       {Ross Girshick and Ilija Radosavovic and Georgia Gkioxari and
                  Piotr Doll\'{a}r and Kaiming He},
  title =        {Detectron},
  howpublished = {\url{https://github.com/facebookresearch/detectron}},
  year =         {2018}
}

@inproceedings{huang2017speed,
  title={Speed/accuracy trade-offs for modern convolutional object detectors},
  author={Huang, Jonathan and Rathod, Vivek and Sun, Chen and Zhu, Menglong and Korattikara, Anoop and Fathi, Alireza and Fischer, Ian and Wojna, Zbigniew and Song, Yang and Guadarrama, Sergio and others},
  booktitle={IEEE CVPR},
  volume={4},
  year={2017}
}

@article{hinton2015distilling,
  title={Distilling the knowledge in a neural network},
  author={Hinton, Geoffrey and Vinyals, Oriol and Dean, Jeff},
  journal={arXiv preprint arXiv:1503.02531},
  year={2015}
}

@inproceedings{szegedy2016rethinking,
  title={Rethinking the inception architecture for computer vision},
  author={Szegedy, Christian and Vanhoucke, Vincent and Ioffe, Sergey and Shlens, Jon and Wojna, Zbigniew},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={2818--2826},
  year={2016}
}

@book{gonzalez2004digital,
  title={Digital image processing using MATLAB.},
  author={Gonzalez, Rafael C and Woods, Richard E and Eddins, Steven L and others},
  volume={624},
  year={2004},
  publisher={Pearson-Prentice-Hall Upper Saddle River, New Jersey}
}

@misc{gonzalez2002digital,
  title={Digital image processing},
  author={Gonzalez, Rafael C and Woods, Richard E and others},
  year={2002},
  publisher={Prentice hall Upper Saddle River, NJ}
}


@inproceedings{feichtenhofer2017detect,
  title={Detect to track and track to detect},
  author={Feichtenhofer, Christoph and Pinz, Axel and Zisserman, Andrew},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={3038--3046},
  year={2017}
}

@inproceedings{wang2018fully,
  title={Fully Motion-Aware Network for Video Object Detection},
  author={Wang, Shiyao and Zhou, Yucong and Yan, Junjie and Deng, Zhidong},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={542--557},
  year={2018}
}
